Stochastic Optimal Control of a Sailboat

In match race sailing, competitors must steer their boats upwind in the presence of unpredictably evolving weather. Combined with the tacking motion necessary to make upwind progress, this makes it natural to model their path-planning as a hybrid stochastic optimal control problem. Dynamic programming provides the tools for solving these, but the computational cost can be significant. We greatly accelerate a semi-Lagrangian iterative approach of Ferretti and Festa (R. Ferretti and A. Festa, "Optimal Route Planning for Sailing Boats: A Hybrid Formulation", J Optim Theory Appl (2019)) by reducing the state space dimension and designing an adaptive timestep discretization that is very nearly causal. We also provide a more accurate tack-switching operator by integrating over potential wind states after the switch. The method is illustrated through a series of simulations with varying stochastic wind conditions.

==> Images/DriftDiff.tex <==
\begin{tikzpicture}[]
\begin{axis}[height = {101.6mm}, ylabel = {$\theta$}, title = {Wind Direction}, xmin = {-0.06000000000000004}, xmax = {2.0600000000000014}, ymax = {0.29765528683462245}, xlabel = {$t$}, unbounded coords=jump,scaled x ticks = false,xlabel style = {font = {\fontsize{11 pt}{14.3 pt}\selectfont}, color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0, rotate = 0.0},xmajorgrids = true,xtick = {0.0,0.5,1.0,1.5,2.0},xticklabels = {$0.0$,$0.5$,$1.0$,$1.5$,$2.0$},xtick align = inside,xticklabel style = {font = {\fontsize{8 pt}{10.4 pt}\selectfont}, color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0, rotate = 0.0},x grid style = {color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000},
draw opacity = 0.1,
line width = 0.5,
solid},axis x line* = left,x axis line style = {color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000},
draw opacity = 1.0,
line width = 1,
solid},scaled y ticks = false,ylabel style = {font = {\fontsize{11 pt}{14.3 pt}\selectfont}, color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0, rotate = 0.0},ymajorgrids = true,ytick = {-0.05,0.0,0.05,0.1,0.15,0.2,0.25},yticklabels = {$-0.05$,$0.00$,$0.05$,$0.10$,$0.15$,$0.20$,$0.25$},ytick align = inside,yticklabel style = {font = {\fontsize{8 pt}{10.4 pt}\selectfont}, color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0, rotate = 0.0},y grid style = {color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000},
draw opacity = 0.1,
line width = 0.5,
solid},axis y line* = left,y axis line style = {color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000},
draw opacity = 1.0,
line width = 1,
solid},    xshift = 0.0mm,
    yshift = 0.0mm,
    axis background/.style={fill={rgb,1:red,1.00000000;green,1.00000000;blue,1.00000000}}
,title style = {font = {\fontsize{14 pt}{18.2 pt}\selectfont}, color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0, rotate = 0.0},legend style = {color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000},
draw opacity = 1.0,
line width = 1,
solid,fill = {rgb,1:red,1.00000000;green,1.00000000;blue,1.00000000},font = {\fontsize{8 pt}{10.4 pt}\selectfont}},colorbar style={title=}, ymin = {-0.07187754789596461}, width = {152.4mm}]\addplot+ [color = {rgb,1:red,0.00000000;green,0.60560316;blue,0.97868012},
draw opacity = 1.0,
line width = 1,
solid,mark = none,
mark size = 2.0,
mark options = {
    color = {rgb,1:red,0.00000000;green,0.00000000;blue,0.00000000}, draw opacity = 1.0,
    fill = {rgb,1:red,0.00000000;green,0.60560316;blue,0.97868012}, fill opacity = 1.0,
    line width = 1,
    rotate = 0,
    solid
},forget plot]coordinates {
(0.0, 0.0)
(0.01, -0.018534916290803075)
(0.02, -0.0035006780576157474)
(0.03, -0.0016758217218850967)
(0.04, 0.0033939488671749203)
(0.05, -0.0020945974599299267)
(0.060000000000000005, -0.005541255925669378)
(0.07, 0.007918271567752298)
(0.08, -0.006462058208417302)
(0.09, -0.00956476155332673)
(0.09999999999999999, -0.004822280832484406)
(0.10999999999999999, -0.013001519261578033)
(0.11999999999999998, -0.018369654807862477)
(0.12999999999999998, -0.022787969416140058)
(0.13999999999999999, -0.009114471229093984)
(0.15, -0.010533753993962235)
(0.16, -0.010419304916187068)
(0.17, -0.006005549597478961)
(0.18000000000000002, -0.014131709116584727)
(0.19000000000000003, -0.028764519389444944)
(0.20000000000000004, -0.036205970229195854)
(0.21000000000000005, -0.0593025407152413)
(0.22000000000000006, -0.05654280779934141)
(0.23000000000000007, -0.06141907144132535)
(0.24000000000000007, -0.04418912662763667)
(0.25000000000000006, -0.036120921388958324)
(0.26000000000000006, -0.03966520841786274)
(0.2700000000000001, -0.04432672307782302)
(0.2800000000000001, -0.027422458168431214)
(0.2900000000000001, -0.038863467214520414)
(0.3000000000000001, -0.03704612648846082)
(0.3100000000000001, -0.029472373036586223)
(0.3200000000000001, -0.04148938287362071)
(0.3300000000000001, -0.04948835428666551)
(0.34000000000000014, -0.04804390518892184)
(0.35000000000000014, -0.027012116777788867)
(0.36000000000000015, -0.03137217523316538)
(0.37000000000000016, -0.03562039700790978)
(0.38000000000000017, -0.03240244770426396)
(0.3900000000000002, -0.03435131840363463)
(0.4000000000000002, -0.03374249890822308)
(0.4100000000000002, -0.031621054087968864)
(0.4200000000000002, -0.017402481272001225)
(0.4300000000000002, -0.019251823679432956)
(0.4400000000000002, -0.01588929526824273)
(0.45000000000000023, -0.008631865705328421)
(0.46000000000000024, -0.019404578003466542)
(0.47000000000000025, -0.01546117311850846)
(0.48000000000000026, -0.015027138920031526)
(0.49000000000000027, -0.011511849871420567)
(0.5000000000000002, -0.012016784692054694)
(0.5100000000000002, 0.015614615517777212)
(0.5200000000000002, 0.0036959816761682977)
(0.5300000000000002, 0.019539774305074663)
(0.5400000000000003, 0.009012193820188011)
(0.5500000000000003, 0.00828340668871901)
(0.5600000000000003, 0.02476338932912838)
(0.5700000000000003, 0.030145122252651882)
(0.5800000000000003, 0.04091027917589208)
(0.5900000000000003, 0.051532340811159254)
(0.6000000000000003, 0.052991352250304866)
(0.6100000000000003, 0.05420548473226412)
(0.6200000000000003, 0.05055262257331852)
(0.6300000000000003, 0.04749864362070845)
(0.6400000000000003, 0.049082546756431096)
(0.6500000000000004, 0.05564767265005268)
(0.6600000000000004, 0.0642098873003708)
(0.6700000000000004, 0.07900688807974031)
(0.6800000000000004, 0.07840467930387564)
(0.6900000000000004, 0.06494264754963713)
(0.7000000000000004, 0.07157952994853166)
(0.7100000000000004, 0.06329558012752413)
(0.7200000000000004, 0.06363387220484923)
(0.7300000000000004, 0.06880736220802704)
(0.7400000000000004, 0.05504511058306268)
(0.7500000000000004, 0.05949610854747544)
(0.7600000000000005, 0.058675980512209826)
(0.7700000000000005, 0.058089484695264204)
(0.7800000000000005, 0.03720535805458193)
(0.7900000000000005, 0.05030944886215424)
(0.8000000000000005, 0.06968903522637535)
(0.8100000000000005, 0.08404570533593814)
(0.8200000000000005, 0.10724507424413504)
(0.8300000000000005, 0.10248273697673677)
(0.8400000000000005, 0.108032802892715)
(0.8500000000000005, 0.10425889649880327)
(0.8600000000000005, 0.091718210539452)
(0.8700000000000006, 0.08787894261443645)
(0.8800000000000006, 0.07379681635676691)
(0.8900000000000006, 0.062034601325689484)
(0.9000000000000006, 0.07384946589869122)
(0.9100000000000006, 0.07780742965873831)
(0.9200000000000006, 0.09080062792843364)
(0.9300000000000006, 0.10917094188501375)
(0.9400000000000006, 0.11797318783896993)
(0.9500000000000006, 0.10888660451331442)
(0.9600000000000006, 0.11818992122417102)
(0.9700000000000006, 0.12378587908619401)
(0.9800000000000006, 0.10956434594262725)
(0.9900000000000007, 0.11224137271097487)
(1.0000000000000007, 0.11029748662385074)
(1.0100000000000007, 0.09953521764508778)
(1.0200000000000007, 0.10994347410526774)
(1.0300000000000007, 0.1081406219108047)
(1.0400000000000007, 0.10051913555606104)
(1.0500000000000007, 0.09625238373227969)
(1.0600000000000007, 0.10366486707207152)
(1.0700000000000007, 0.11068517395596564)
(1.0800000000000007, 0.10941201500590003)
(1.0900000000000007, 0.10558757394302765)
(1.1000000000000008, 0.09615853209926314)
(1.1100000000000008, 0.09733682589051379)
(1.1200000000000008, 0.10282429397382647)
(1.1300000000000008, 0.1046162937150857)
(1.1400000000000008, 0.11074597980092754)
(1.1500000000000008, 0.11686189834339075)
(1.1600000000000008, 0.12116338407488095)
(1.1700000000000008, 0.11933696903059579)
(1.1800000000000008, 0.12281253840398396)
(1.1900000000000008, 0.12335340331191144)
(1.2000000000000008, 0.1477100777569907)
(1.2100000000000009, 0.14528397406356533)
(1.2200000000000009, 0.15190860658759286)
(1.2300000000000009, 0.1459649069621481)
(1.2400000000000009, 0.11783461848885475)
(1.2500000000000009, 0.12648523131317504)
(1.260000000000001, 0.1322498687448356)
(1.270000000000001, 0.13260913761741605)
(1.280000000000001, 0.12796917973965927)
(1.290000000000001, 0.1336846128622191)
(1.300000000000001, 0.12543756355199864)
(1.310000000000001, 0.11645726729057784)
(1.320000000000001, 0.10798356180357464)
(1.330000000000001, 0.11923680948616325)
(1.340000000000001, 0.12577127019309953)
(1.350000000000001, 0.1279522251194223)
(1.360000000000001, 0.12427422220591625)
(1.370000000000001, 0.12650866316410733)
(1.380000000000001, 0.11738525966540123)
(1.390000000000001, 0.12097189073684772)
(1.400000000000001, 0.12518059485414365)
(1.410000000000001, 0.12728863151379444)
(1.420000000000001, 0.11458819036784143)
(1.430000000000001, 0.09684068563495557)
(1.440000000000001, 0.10517002370130007)
(1.450000000000001, 0.11079393996808906)
(1.460000000000001, 0.10260907992245583)
(1.470000000000001, 0.11758790838854769)
(1.480000000000001, 0.12189473996699356)
(1.490000000000001, 0.1270480244511532)
(1.500000000000001, 0.12226404895936711)
(1.5100000000000011, 0.14123067089653352)
(1.5200000000000011, 0.1330640140563644)
(1.5300000000000011, 0.13952720804849672)
(1.5400000000000011, 0.14273530211935553)
(1.5500000000000012, 0.1545120231649513)
(1.5600000000000012, 0.15441757227858494)
(1.5700000000000012, 0.1615024321514645)
(1.5800000000000012, 0.16547928473661616)
(1.5900000000000012, 0.1771543633477283)
(1.6000000000000012, 0.17483904087061344)
(1.6100000000000012, 0.18701929160606232)
(1.6200000000000012, 0.19444247615201551)
(1.6300000000000012, 0.21412933959741343)
(1.6400000000000012, 0.22445935407131154)
(1.6500000000000012, 0.21477967704168924)
(1.6600000000000013, 0.2231578599588007)
(1.6700000000000013, 0.22311786052801816)
(1.6800000000000013, 0.23154329849852592)
(1.6900000000000013, 0.2387261504283944)
(1.7000000000000013, 0.24269212358592113)
(1.7100000000000013, 0.25197071893551953)
(1.7200000000000013, 0.24201934352978444)
(1.7300000000000013, 0.2446908198490895)
(1.7400000000000013, 0.2607337816456824)
(1.7500000000000013, 0.2697135833903015)
(1.7600000000000013, 0.2556272226230243)
(1.7700000000000014, 0.2369007348446314)
(1.7800000000000014, 0.24428150473014196)
(1.7900000000000014, 0.23560298311947914)
(1.8000000000000014, 0.23765739477840475)
(1.8100000000000014, 0.23474872692089047)
(1.8200000000000014, 0.22660566185367154)
(1.8300000000000014, 0.2411565693553669)
(1.8400000000000014, 0.23339903288071667)
(1.8500000000000014, 0.23835215866191484)
(1.8600000000000014, 0.2334279972943746)
(1.8700000000000014, 0.241574883091939)
(1.8800000000000014, 0.24020174760885035)
(1.8900000000000015, 0.2515600224465399)
(1.9000000000000015, 0.2499569814772025)
(1.9100000000000015, 0.2556618280280723)
(1.9200000000000015, 0.2625026297280311)
(1.9300000000000015, 0.26723388152056876)
(1.9400000000000015, 0.2659571877553941)
(1.9500000000000015, 0.26462454747820674)
(1.9600000000000015, 0.26190353639882086)
(1.9700000000000015, 0.24348855575401693)
(1.9800000000000015, 0.26127549664566707)
(1.9900000000000015, 0.2714920284419799)
(2.0000000000000013, 0.2871968103799832)
};
\end{axis}

\end{tikzpicture}


==> error_scaling.tex <==
Next, we perform an error refinement analysis by running our algorithm over progressively finer grids. Taking the values of the grid points of the finest grid using standard Gauss-Seidel iteration as ``ground truth'', we measure the average $l_1$ and $l_\infty$ norms of the shared points in the coarser grids and observe how these grow as the grid is coarsened. These plots can be seen for a variety of values of $\sigma, a$ in Figs.\ \ref{fig_refine_l1} and \ref{fig_refine_linf}. Though the x-axis is just labeled $\Delta r$, both $\Delta r$ and $\Delta \theta$ are refined by the same factors at each point (a division by $2$). The black line in each plot is the slope 1 line.

We can see that on the whole, row-wise Gauss-Seidel has a noticably higher error than standard Gauss-Seidel iteration, and that this error gap increases with the drift parameter $a$. However, both average $l_1$ errors decrease roughly linearly with $\Delta r$, and since the row-wise Gauss-Seidel discretization is roughly $100$ times faster, we may be able to obtain a more accurate solution in the same computation time by using an even finer grid.

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
            \resizebox{\textwidth}{!}{
            \input{Images/RefineL1Comp_σ0.0_D0.0}
        }
        \caption{$\sigma = 0.0, a = 0.0$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \input{Images/RefineL1Comp_σ0.1_D0.0}
        }
        \caption{$\sigma = 0.1, a = 0.0$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \input{Images/RefineL1Comp_σ0.05_D0.1}
        }
        \caption{$\sigma = 0.05, a = 0.1$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \input{Images/RefineL1Comp_σ0.05_D0.15}
        }
        \caption{$\sigma = 0.05, a = 0.15$}
    \end{subfigure}
    \caption{Measurements of the average $l_1$ error under refinement of the grid.}
    \label{fig_refine_l1}
\end{figure}

A more worrying observation is the behavior of the $l_\infty$ norm. We can see that in this norm, the row-wise Gauss-Seidel method begins to plateau at fine grid scales. The fact that the $l_\infty$ norm behavior is so radically different than the average $l_1$ norm behavior indicates that the error is not uniform over the grid. There are local areas of the domain where the algorithm is doing much worse than average, and these areas are starting to cease to improve as the grid is refined.

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
            \resizebox{\textwidth}{!}{
            \input{Images/RefineLInfComp_σ0.0_D0.0}
        }
        \caption{$\sigma = 0.0, a = 0.0$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \input{Images/RefineLInfComp_σ0.1_D0.0}
        }
        \caption{$\sigma = 0.1, a = 0.0$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \input{Images/RefineLInfComp_σ0.05_D0.1}
        }
        \caption{$\sigma = 0.05, a = 0.1$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
            \input{Images/RefineLInfComp_σ0.05_D0.15}
        }
        \caption{$\sigma = 0.05, a = 0.15$}
    \end{subfigure}
    \caption{Measurements of the average $l_\infty$ error under refinement of the grid.}
    \label{fig_refine_linf}
\end{figure}

To investigate this, in Fig.\ \ref{fig_errmap_normal} and \ref{fig_errmap_fast} we plot the error at different points in the domain for both the standard and row-wise Gauss-Seidel iterations. All errors are averaged across both tacks $q=1,2$. A number of interesting patterns emerge. {\color{red} Something insightful here...}

In both cases, we can see that there are small number of points right on the edge of the target which carry a high level of error. These points seem to be consistent across both discretizations and various parameter values. However, the level of error in these points is much more pronounced in the row-wise iterations. It seems that these points are responsible for the plateau seen in the $l_\infty$ error plots. Though, there are very distinct local error patterns elsewhere in each plot.

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/ErrMap_σ00_D00.png}
        \caption{$\sigma = 0.0, a = 0.0$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/ErrMap_σ01_D00.png}
        \caption{$\sigma = 0.1, a = 0.0$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/ErrMap_σ005_D005.png}
        \caption{$\sigma = 0.05, a = 0.05$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/ErrMap_σ005_D015.png}
        \caption{$\sigma = 0.05, a = 0.15$}
    \end{subfigure}
    \caption{Error Maps for normal Gauss-Seidel iterations}
    \label{fig_errmap_normal}
\end{figure}

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/FastErrMap_σ00_D00.png}
        \caption{$\sigma = 0.0, a = 0.0$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/FastErrMap_σ01_D00.png}
        \caption{$\sigma = 0.1, a = 0.0$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/FastErrMap_σ005_D005.png}
        \caption{$\sigma = 0.05, a = 0.05$}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Images/FastErrMap_σ005_D015.png}
        \caption{$\sigma = 0.05, a = 0.15$}
    \end{subfigure}
    \caption{Error Maps for row-wise Gauss-Seidel iterations}
    \label{fig_errmap_fast}
\end{figure}

==> fast_convergence.tex <==
In Fig.\ \ref{fig_sweep_perf}, we show the number of iterations required to achieve convergence for our various discretizations on an example problem. As shown, row-wise Gauss-Seidel iteration requires a nearly-constant number of iterations, only slowly beginning to increase at large granularities. Meanwhile, both Gauss-Jacobi and standard Gauss-Seidel discretizations require a number of iterations roughly linear in the number of grid points. At the largest grid size tested, Gauss-Jacobi requires a factor of $\approx100$ more iterations than Gauss-Seidel, which itself requires a factor of $\approx100$ more iterations than row-wise Gauss-Seidel.

However, this massive speedup by using row-wise Gauss-Seidel iteration is not completely free. Comparing Eqs.\ \ref{eq_adaptivedt} and \ref{eq_row-wisedt}, we can see that row-wise iteration uses timesteps which are larger than the standard discretization in areas of the domain where $\Delta \theta / \dot{\theta} < \Delta r / \dot{r}$, in particular close to the target. We provide extended error analysis measurements online at \url{urlhere}, finding the global errors to be slightly larger, but decreasing at same rate for all discretizations at large granularities.

